ProAct: Progressive Training for Hybrid Clipped Activation Function to Enhance Resilience of DNNs

Deep Neural Networks (DNNs) are extensively employed in safety-critical applications where ensuring hardware reliability is a primary concern. To enhance the reliability of DNNs against hardware faults, activation restriction techniques significantly mitigate the fault effects at the DNN structure level, irrespective of accelerator architectures. State-of-the-art methods offer either neuron-wise or layer-wise clipping activation functions. They attempt to determine optimal clipping thresholds using heuristic and learning-based approaches. Layer-wise clipped activation functions cannot preserve DNNs resilience at high bit error rates. On the other hand, neuron-wise clipping activation functions introduce considerable memory overhead due to the addition of parameters, which increases their vulnerability to faults. Moreover, the heuristic-based optimization approach demands numerous fault injections during the search process, resulting in time-consuming threshold identification. On the other hand, learning-based techniques that train thresholds for entire layers concurrently often yield sub-optimal results. In this work, first, we demonstrate that it is not essential to incorporate neuron-wise activation functions throughout all layers in DNNs. Then, we propose a hybrid clipped activation function that integrates neuron-wise and layer-wise methods that apply neuron-wise clipping only in the last layer of DNNs. Additionally, to attain optimal thresholds in the clipping activation function, we introduce ProAct, a progressive training methodology. This approach iteratively trains the thresholds on a layer-by-layer basis, aiming to obtain optimal threshold values in each layer separately.

==> Src/Help.tex <==
% \begin{table*}[hbpt]
% \captionsetup{justification=centering}
% \begin{center}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{ccc}
% \resizebox{\columnwidth}{!}{
%   \begin{tikzpicture}
%     \begin{axis}[every axis plot post/.append style={
%       mark=none,domain=-20:200,samples=1000,smooth},
%       font=\small,
%         ybar=0.06cm,
%         width=\columnwidth,
%      height=0.63\columnwidth,
%      ylabel near ticks,
%     xlabel near ticks,
%     ymin=0, ymax=0.5,
%     ylabel= \textbf{\large Density},
%     xlabel= \textbf{\large Values},
%     enlarge x limits=0.03,
%     legend style={at={(0.75,1)},
%     anchor=north,legend columns=-1, font=\fontsize{10}{5}\selectfont},
%      grid=major,
%             grid style={dashed,gray!70},
%         % 	xtick=data,
%         % 	extra y ticks={-5,5,15},
% 	        nodes near coords align={vertical},
%         	bar width=2.5pt] 
%   \addplot [
%         fill opacity=1,
%         fill=green,
%         draw=green,
%         hist=density
%     ] table  [x=x, y=y, col sep=comma] {Figs/data_density_orig.csv};
%     \addplot [
%     fill opacity=0.3,
%         fill=blue,
%         draw=blue,
%         hist=density
%     ] table  [x=x, y=y, col sep=comma] {Figs/data_density_ftclip.csv};
%     % \addplot [
%     % fill opacity=0.4,
%     %     fill=violet,
%     %     draw=violet,
%     %     hist=density
%     % ] table  [x=x, y=y, col sep=comma] {Figs/data_density_fitact.csv};
%     % \addplot [
%     % fill opacity=0.4,
%     %     fill=red,
%     %     draw=red,
%     %     hist=density
%     % ] table  [x=x, y=y, col sep=comma] {Figs/data_density_redact.csv};
%     \legend{Fault-free, FT-ClipAct}
%     \end{axis}
    
%     \end{tikzpicture}}
%     &
%      \begin{tikzpicture}
%     \begin{axis}[every axis plot post/.append style={
%       mark=none,domain=-20:200,samples=1000,smooth},
%       font=\small,
%         ybar=0.06cm,
%         width=\columnwidth,
%      height=0.63\columnwidth,
%      ylabel near ticks,
%     xlabel near ticks,
%     ymin=0, ymax=0.5,
%     ylabel= \textbf{{ \large Density}},
%     xlabel= \textbf{{ \large Values}},
%     enlarge x limits=0.03,
%     legend style={at={(0.79,1)},
%     anchor=north,legend columns=-1, font=\fontsize{10}{5}\selectfont},
%      grid=major,
%             grid style={dashed,gray!70},
%         % 	xtick=data,
%         % 	extra y ticks={-5,5,15},
% 	        nodes near coords align={vertical},
%         	bar width=2.5pt] 
%   \addplot [
%         fill opacity=1,
%         fill=green,
%         draw=green,
%         hist=density
%     ] table  [x=x, y=y, col sep=comma] {Figs/data_density_orig.csv};
%     % \addplot [
%     % fill opacity=0.3,
%     %     fill=blue,
%     %     draw=blue,
%     %     hist=density
%     % ] table  [x=x, y=y, col sep=comma] {Figs/data_density_ftclip.csv};
%     \addplot [
%     fill opacity=0.4,
%         fill=violet,
%         draw=violet,
%         hist=density
%     ] table  [x=x, y=y, col sep=comma] {Figs/data_density_fitact.csv};
%     % \addplot [
%     % fill opacity=0.4,
%     %     fill=red,
%     %     draw=red,
%     %     hist=density
%     % ] table  [x=x, y=y, col sep=comma] {Figs/data_density_redact.csv};
%     \legend{Fault-free,FitAct}
%     \end{axis}
    
%     \end{tikzpicture}
%     &
%     \begin{tikzpicture}
%     \begin{axis}[every axis plot post/.append style={
%       mark=none,domain=-20:200,samples=1000,smooth},
%       font=\small,
%         ybar=0.06cm,
%         width=\columnwidth,
%      height=0.63\columnwidth,
%      ylabel near ticks,
%     xlabel near ticks,
%     ymin=0, ymax=0.5,
%     ylabel=\textbf{ {\large Density}},
%     xlabel=\textbf{{\large Values}},
%     enlarge x limits=0.03,
%     legend style={at={(0.78,1)},
%     anchor=north,legend columns=-1, font=\fontsize{10}{5}\selectfont},
%      grid=major,
%             grid style={dashed,gray!70},
%         % 	xtick=data,
%         % 	extra y ticks={-5,5,15},
% 	        nodes near coords align={vertical},
%         	bar width=2.5pt] 
%   \addplot [
%         fill opacity=1,
%         fill=green,
%         draw=green,
%         hist=density
%     ] table  [x=x, y=y, col sep=comma] {Figs/data_density_orig.csv};
%     % \addplot [
%     % fill opacity=0.3,
%     %     fill=blue,
%     %     draw=blue,
%     %     hist=density
%     % ] table  [x=x, y=y, col sep=comma] {Figs/data_density_ftclip.csv};
%     % \addplot [
%     % fill opacity=0.4,
%     %     fill=violet,
%     %     draw=violet,
%     %     hist=density
%     % ] table  [x=x, y=y, col sep=comma] {Figs/data_density_fitact.csv};
%     \addplot [
%     fill opacity=0.4,
%         fill=red,
%         draw=red,
%         hist=density
%     ] table  [x=x, y=y, col sep=comma] {Figs/data_density_redact.csv};
%     \legend{Fault-free, RedAct}
%     \end{axis}
    
%     \end{tikzpicture}
%      \\
%      \;\;\;\;\;\;\;\;\;\;\;\;      \large \textbf{(a)} & \;\;\;\;\;\;\;\;\;\;\;\;      \large \textbf{(b)} & \;\;\;\;\;\;\;\;\;\;\;\;      \large \textbf{(c)}  
    
%     % \includegraphics[width = 0.9\columnwidth]{Figs/fc3_motivation.pdf}
% \end{tabular}}
% \end{center}
% \captionof{figure}{Comparing the ratio of 0 value in the activations of fault-free AlexNet's FC3 layer, with faulty one at $1E-4$ fault-rate applying a) FT-ClipAct, b) FitAct, and c) Red-Act.}
% \label{fig:non-zero-results}
% \end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%
\begin{comment}
\begin{figure}[t]
\captionsetup{justification=centering}
\resizebox{\columnwidth}{!}{
  \begin{tikzpicture}
        \begin{axis}[
            ybar=0.06cm,
            ymin =0.55, ymax=1.0,
        	symbolic x	coords={conv1,conv2,conv3,conv4,conv5,fc1,fc2,fc3},
        	width=\columnwidth,
            height=0.6\columnwidth,
            ylabel near ticks,
            xlabel near ticks,
            grid=major,
            grid style={dashed,gray!70},
        	ylabel= \textbf{\scriptsize Density of zero elements},
        	xlabel= \textbf{\scriptsize Layer},
        % 	enlargelimits=0.15,
        	tick label style={font=\small},  
        	enlarge x limits=0.03,
        	legend style={at={(0.5,1.17)},
        		anchor=north,legend columns=-1, font=\fontsize{8}{5}\selectfont},
        	xtick=data,
        % 	extra y ticks={-5,5,15},
	        nodes near coords align={vertical},
        	bar width=1.8pt
        ]
        \addplot [green!70, fill] % 
        	coordinates {(conv1,0.7393931518554687) (conv2,0.8590656875) (conv3,0.8951954895833333) (conv4,0.918140828125) (conv5,0.86910546875) (fc1,0.6819916748046875) (fc2,0.7105964111328125) (fc3,0.59865) };
        \addplot [blue, fill] % 
        	coordinates {(conv1,0.7497855834960937) (conv2,0.8808094947916667) (conv3,0.9324786979166667) (conv4,0.941825515625) (conv5,0.892500265625) (fc1,0.76584921875) (fc2,0.9188308837890625) (fc3,0.88367) };
         
          \addplot [violet, fill] % 
        	coordinates {(conv1,0.7453) (conv2,0.8701) (conv3,0.9184) (conv4,0.9292) (conv5,0.8812) (fc1,0.7431) (fc2,0.8834) (fc3,0.8432) };  	
        \addplot [red, fill] % 
        	coordinates {(conv1,0.73939484252929) (conv2,0.8605127708333333) (conv3,0.8932494791666666) (conv4,0.918408359) (conv5,0.86787784375) (fc1,0.68518076171875) (fc2,0.711535278320) (fc3,0.59508) }; 
        \legend{Fault-free, FtClipAct, FitAct,ReD-Act}
        \end{axis}
    \end{tikzpicture}}
\caption{Ratio of 0 value in the activations of different layers of AlexNet in fault-free unprotected, faulty FT-ClipAct, and faulty ReD-Act (fault rate = $10^{-4}$).}
\label{fig:method:numzero}
\end{figure}

\end{comment}
